Distributions of missing sums and differences

This paper discusses the distributions of missing sums and differences.

==> approach.tex <==
\section{Approach}

\begin{figure}[tb!]
  \centering
  \subfloat[Vector input]
  	{\label{fig:whale_input}
  	\includegraphics[height=0.11\textwidth]
  	{whale_input.pdf}}
  \subfloat[Illustrator]
  	{\label{fig:whale_illustrator}
  	\includegraphics[height=0.11\textwidth]
  	{whale_illustrator.pdf}}
  \subfloat[Photoshop]
  	{\label{fig:whale_photoshop}
  	\includegraphics[height=0.11\textwidth]
  	{whale_photoshop.pdf}}
  \subfloat[Pixelation]
  	{\label{fig:whale_pixelator}
  	\includegraphics[height=0.11\textwidth]
  	{whale_pixelator.pdf}}
  	\caption{Computer-generated pixel art drawings.
  	}
  	\label{fig:compare}
\end{figure}

%\begin{figure}[tb!]
%  \centering
%  	\includegraphics[height=0.9\textwidth]
%  	{skull600_200_type5_square.png}
%  	\caption{A skull rendered in the hybrid Op Art style.}
%  \label{fig:hybrid}
%\end{figure}

To pixelate a curve, it is first divided into smooth monotonic curve segments. For each curve segment, we use a greedy algorithm to compute a piecewise polygonal approximation in which the slope of each line segment is of the form $n$ or $1/n$, where $n$ is a positive integer. Then each line segment is replaced by either a column or a row of pixels to obtain the pixelated curve corresponding to the curve segment.

The basic algorithm we just described may produce jagged curves. To remove jaggies, shift the curve segments so that they are better aligned with the pixel grid, and then the final pixelated curve is checked for slope monotonicity. For example, if a vector curve is monotonically increasing in slope, then the pixels in the corresponding pixelated curve are rearranged to reflect this property.

To evaluate our Pixelation algorithm, a two-part user study was conducted. In Part 1, participants were given eight vector images, each superimposed on a pixel grid, and their task was to draw the corresponding pixel art. In Part 2, we merged the participants' drawings with results generated by our algorithm as well as Adobe Illustrator and Adobe Photoshop (see Figure~\ref{fig:compare}). Participants were then presented with pairs of pixel drawings and asked to choose which they preferred based on visual appeal and fidelity.

According to the results, our algorithm significantly outperformed both Adobe Illustrator and Photoshop. We analyzed the highest rated drawings from artists and learned that being able to interpret and understand the input image is very important to creating good pixel art drawings. For example, in Figure~\ref{fig:compare}, we know the eye should be round. Therefore, we try to draw it as a circle, even if it involves some shifting and rescaling.

For future work, we are interested in developing techniques for other aspects of pixel art such as selecting relevant features to include based on the resolution, choosing a suitable colour palette, applying manual dithering and anti-aliasing, and creating isometric pixel art from 3D models.

==> dstribution.tex <==
\section{Relating several distributions for number of missing sums}

Knowing the probability
$\Prob{k \in \Rinf + \Rinf | k-1 \in \Rinf + \Rinf}$
is only the tip of the iceberg. What we are really aiming to find out is, for any $n \geq 0$, how $R_n + R_n$ varies in size. Certainly, $\{R_n + R_n\}$
